Dynamic Page Placement on Real Persistent Memory Systems

As persistent memory (PM) technologies emerge, hybrid memory architectures combining DRAM with PM bring the potential to provide a tiered, byte-addressable main memory of unprecedented capacity. Nearly a decade after the first proposals for these hybrid architectures, the real technology has finally reached commercial availability with Intel Optane(TM) DC Persistent Memory (DCPMM). This raises the challenge of designing systems that realize this potential in practice, namely through effective approaches that dynamically decide at which memory tier should pages be placed. In this paper, we are the first, to our knowledge, to systematically analyze tiered page placement on real DCPMM-based systems. To this end, we start by revisiting the assumptions of state-of-the-art proposals, and confronting them with the idiosyncrasies of today's off-the-shelf DCPMM-equipped architectures. This empirical study reveals that some of the key design choices in the literature rely on important assumptions that are not verified in present-day DRAM-DCPMM memory architectures. Based on the lessons from this study, we design and implement HyPlacer, a tool for tiered page placement in off-the-shelf Linux-based systems equipped with DRAM+DCPMM. In contrast to previous proposals, HyPlacer follows an approach guided by two main practicality principles: 1) it is tailored to the performance idiosyncrasies of off-theshelf DRAM+DCPMM systems; and 2) it can be seamlessly integrated into Linux with minimal kernel-mode components, while ensuring extensibility to other HMAs and other data placement policies. Our experimental evaluation of HyPlacer shows that it outperforms both solutions proposed in past literature and placement options that are currently available in off-the-shelf DCPMM-equipped Linux systems, reaching an improvement of up to 11x when compared to the default memory policy in Linux.

==> implementation_old.tex <==
\section{\name \jpb{old version, probably longer, for us to check if any relevant bit should be moved to the main version}}
\label{section:implementation}

\name manages page placement within a socket with a DRAM and ADM \optane tiers, illustrated in \Cref{subfig:optane-adm-arch}.
Our solution requires minimal changes to the Linux kernel, and expands existing page placement mechanisms in order to accommodate the integration of \optane.
\name leverages: (i)~existing page walking mechanisms, (ii)~the page table's dirty and reference bits, managed by the memory management unit (MMU), (iii)~the \textit{move\_pages} syscall in order to migrate pages between tiers, and (iv)~Processor Counter Monitor (PCMon) \cite{pcmon}, which allows \name to determine the bandwidth usage of each of the memories with hardware counters available in most modern Intel CPUs.

Our solution combines the collected page and bandwidth metrics at runtime in order to perform page placement decisions that take advantage of each tier's characteristics, and ultimately improve throughput by several times compared to a default allocation policy.


Following the insights provided in \Cref{section:optane-tailoring}, \name separates pages into three different categories: write-intensive, read-intensive and cold.
The algorithm keeps as many write-intensive pages as possible in DRAM.
If these do not fully occupy DRAM, the solution prefers read-intensive over cold pages in the faster tier.

\noindent \name periodically determines the suitability of the current page distribution, measured in terms of the following three criteria:
\begin{itemize}
    \item DRAM has enough free space to allow newly referenced pages to fit in the faster tier.
    These pages are expected to be accessed frequently after allocated, due to the \emph{temporal locality} principle.
    To this end, \name maintains a defined buffer of free space in DRAM by demoting pages eagerly, before it is depleted;
    \item \optane's write throughput is nominal, indicating that the tier does not contain a significant amount of frequently modified pages;
    \item If DRAM is at capacity but the \optane's write threshold is substantial, no pages can be exchanged between both tiers, such that the threshold is reduced.
\end{itemize}

If the current distribution does not meet any of these criteria, \name devises a new placement decision that corrects it, migrating a subset of pages in a given orientation.

In order to select which pages to migrate, \name leverages unmodified page table walk (pagewalk) and PTE bit manipulation mechanisms, implemented in the Linux kernel.
These mechanisms have a relatively stable implementation, which benefits \name by making it compatible with a wide range of kernel versions.
Furthermore, configuring \name on a new kernel version requires only a single line of code, which exports the pagewalk routine, making it available to our solution.

In demotion scenarios, we apply concepts from the traditional CLOCK algorithm, modified to separate intensive pages into read- and write-dominated.
Page promotion, on the other hand, applies a novel \comp{delay} mechanism, which allows \name to identify recently accessed and modified pages in the \optane tier with low overhead.

\name also implements an exchange-based migration technique, using only pre-existing system calls, wherein an equal number of pages are switched between both tiers, thus preserving their current allocation.

In order to monitor multiple sockets, different instances of \name must be launched, each targeting a single socket.
For simplicity of presentation, the following sections assume a single-socket scenario, where only one instance of \name runs.

\subsection{Architecture}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{Figures/ambix-architecture.pdf}
  \caption{\name architecture overview.}
  \label{fig:architecture}
\end{figure}

\Cref{fig:architecture} provides an overview of \name, presenting its components and how they interact.
Our solution consists of two main components: \comp{Control} and the Page Selection Module (\comp{SelMo}).

\comp{Control} is an elevated process running in user-space, which is responsible for formulating and putting into effect new placement decisions, and binding/unbinding applications to our solution.
In order to formulate new decisions, the component leverages Processor Counter Monitor (\comp{PCMon})~\cite{pcmon}, which periodically outputs the current throughput per node to a shared text file.

To use kernel-implemented mechanisms, \name integrates a kernel-space module, named \comp{SelMo}.
The module selects pages belonging to bound processes, in order to carry out the \comp{Control}'s decisions.

The dual-component implementation achieves a small footprint in kernel-space, since all mechanisms related to devising and effectuating new placement decisions are offloaded to the user-space component.

\subsection{Implementation}

\comp{Control} periodically monitors current memory usage and throughput values per NUMA node. %throughput / data rate
It is also able to detect the presence of write-intensive pages in \optane, without communicating with \comp{SelMo}, by reading the information file generated by \comp{PCMon}.

Depending on the collected metrics, \comp{Control} devises a new placement decision and sends a \comp{PageFind} request to \comp{SelMo}.
The request contains the number of pages to find and specifies the selection criteria, or mode.

\begin{table}[t]
\caption{\label{tab:find} \comp{PageFind} modes and goal.}
\scriptsize
 \begin{tabulary}{\linewidth}{| C | C | C |} 
 \hline
 \textbf{Mode} & \textbf{Tier Scope} & \textbf{Goal} \\
 \hline\hline
 \comp{DEMOTE} & DRAM & Demote cold pages \\ 
 \hline
 \comp{PROMOTE} & \optane & Promote pages \\
 \hline
 \comp{PROMOTE\_INT} & \optane & Promote only intensive pages \\
 \hline
 \comp{SWITCH} & Bidirectional & Switch intensive with cold pages \\
 \hline
 \comp{DCPMM\_CLEAR} & \optane & Clear the R/D bits from all resident pages \\
 \hline
\end{tabulary}
\end{table}


In \Cref{tab:find} we summarize the multiple modes, describing the tier from which they select pages, and their respective goals.

By design, DRAM has a defined maximum usage threshold below its actual size.
Above the threshold, \name considers that the tier is full or near depletion, and requests DRAM-resident cold pages to demote from \comp{SelMo}, via a \comp{DEMOTE PageFind}.

Similarly, \optane has a defined write throughput threshold.
If \optane's current throughput is above the defined threshold, \comp{Control} requests intensive pages and promotes them to DRAM.
If DRAM is above its usage threshold, an equal number of pages must be demoted, such that the free space buffer is preserved.
Therefore, a \comp{SWITCH PageFind} is sent to the module.
Otherwise, it tries to maximize the faster tier's utilization, by promoting as many intensive pages as possible such that the usage threshold is not surpassed, by requesting a \comp{PROMOTE\_INT PageFind}.

Inversely, if the \optane's throughput is below its threshold, two decisions can be performed.
If DRAM has enough available space, \comp{Control} allows cold pages to be eagerly promoted, via a \comp{PROMOTE PageFind}.
Otherwise, if DRAM is near depletion, a \comp{DEMOTE PageFind} is requested, such that cold pages are demoted.

Before sending any \comp{PageFind} request that will promote pages, \comp{Control} requests \comp{SelMo} to clear the R/D bits of all PTEs pointing to pages in the \optane tier, via the \comp{DCPMM\_CLEAR PageFind}, after which it waits for a configurable \comp{delay}.

\comp{Delay} affects the access frequency at which a page is considered intensive.
Pages that are accessed or modified during the \comp{delay} interval are considered read- or write-intensive, while all others are classified as cold.

After receiving a \comp{PageFind} request, \comp{SelMo} iterates over each bound process' page table, in order to select which pages \comp{Control} should migrate.

The module leverages the kernel-implemented \code{walk\_page\_range()} routine, which iterates over a defined virtual address range.
\comp{SelMo} passes a PTE callback as an argument to the routine, so that it can observe and manipulate each PTE's R/D bits. 
Since we want to perform different operations depending on the goal of the \comp{PageFind} request, we define multiple callbacks, one for each mode.

If the callback's goal is to demote pages, then it clears the R/D bits of all pages that are not selected to demote.
If one such page is referenced thereafter, the memory management unit (MMU) sets its PTE's \textit{reference} bit; and also its \textit{modified} bit, in the event of a store operation.
In contrast, if the page is not accessed until the next page table iteration, then it is suitable for demotion.

If, on the other hand, the callback's goal is to promote pages, then PTEs are expected to have both \textit{R/D} bits unset, since they have been recently cleared by the module.
In this scenario, the MMU may change the PTE's R/D bits, so that the respective page is suitable for promotion over a next page table iteration.
Therefore, promotion callbacks do not directly manipulate R/D bits.
Instead, the algorithm deems a page in the \optane intensive if referenced during the \comp{delay} window, and write-dominated if modified.

When: (i) the number of selected pages exceeds the required amount set in the request; or (ii) the process has iterated over all PTEs, the page selection phase ends.
At this point, the last PTE's address and PID is stored and the page selection phase ends.
For each tier, the module keeps two last address and PID pairs, which set the start of the next page selection phase for that tier.
Thus, PTEs that have not been inspected for longer are prioritized for migration over recently seen ones.

Then, a reply-back phase begins, where \comp{SelMo} prepares a final page array to be sent back to \comp{Control}, containing all selected pages, after which the latter migrates them.
